Ego-R1: Chain-of-Tool-Thought for Ultra-Long Egocentric Video Reasoning

We introduce Ego-R1, a novel framework for reasoning over ultra-long (i.e., in days and weeks) egocentric videos, which leverages a structured Chain-of-Tool-Thought (CoTT) process, orchestrated by an Ego-R1 Agent trained via reinforcement learning (RL). Inspired by human problem-solving strategies, CoTT decomposes complex reasoning into modular steps, with the RL agent invoking specific tools, one per step, to iteratively and collaboratively answer sub-questions tackling such tasks as temporal retrieval and multi-modal understanding. We design a two-stage training paradigm involving supervised finetuning (SFT) of a pretrained language model using CoTT data and RL to enable our agent to dynamically propose step-by-step tools for long-range reasoning. To facilitate training, we construct a dataset called Ego-R1 Data, which consists of Ego-CoTT-25K for SFT and Ego-QA-4.4K for RL. Furthermore, our Ego-R1 agent is evaluated on a newly curated week-long video QA benchmark, Ego-R1 Bench, which contains human-verified QA pairs from hybrid sources. Extensive results demonstrate that the dynamic, tool-augmented chain-of-thought reasoning by our Ego-R1 Agent can effectively tackle the unique challenges of understanding ultra-long egocentric videos, significantly extending the time coverage from few hours to a week.

==> tabs/qualitative_example.tex <==
% \begin{tcolorbox}[enhanced, breakable, title=Video-R1]
%     <think>Let me think about this for a moment. The question is asking about what I am assembling for the first time. Now, let's break it down and consider each option carefully.  A. Hard drive - A hard drive is a component of a computer. While it's a crucial part, it's not typically assembled by the average person. It's usually pre-assembled and sold as a unit.  B. Computer - A computer is a complex device that consists of various components. It's not something that is typically assembled by the average person. It's usually assembled by professionals or advanced users.  C. Monitor - A monitor is a display device. While it's an important part of a computer, it's not typically assembled by the average person. It's usually sold as a complete unit.  D. Keyboard - A keyboard is a peripheral device. While it's an important part of a computer, it's not typically assembled by the average person. It's usually sold as a complete unit.  Hmm, it seems that the most logical option is the one that involves assembling a complex device that requires multiple components. The computer is the most complex and requires the assembly of various parts.   Oh, I see. The question is asking about the first time assembling something, and the computer is the most complex and requires the most assembly. Therefore, the answer should be the computer.  Let's verify this one more time. The computer is the most complex and requires the most assembly, which aligns with the question's context.  Final answer: B  Let's break it down one last time to ensure. The computer is the most complex and requires the most assembly, which is the most logical answer.</think> <answer>B</answer>
% \end{tcolorbox}


% \begin{tcolorbox}[enhanced, breakable, title=Ego-R1]
% <think>To answer "What am I assembling the first time I assemble something?" at DAY4 \_17091712, I need to determine:
% 1. The first instance of assembly by the user before or around this timestamp.
% 2. What object was assembled during that first instance.

% tep-by-step plan:
% - First, use the rag tool at the "week" and possibly "day" level to search for assembly-related activities (keywords: "assemble," "assembly," "build," "install") in the logs leading up to DAY4\_17091712. This will help identify when and what the user's first assembly event was.
% - Once I identify the time and context of the first assembly, I will narrow down to the relevant hour or minute using the "rag" tool to clarify what specifically was being assembled.
% - If assembly events are ambiguous, I will use video\_llm to clarify the visual content around the event.
% - Finally, I will use vlm to confirm details of the object assembled at the timestamp, if necessary.

% Let's begin by searching for assembly activities using rag at the week level starting from the beginning up to DAY4\_17091712.</think>


% \begin{verbatim}
% <tool>
% {'name': 'rag',
%     'arguments': '{
%     "level":"week",
%     "keywords":["assemble","assembly","build","install"],
%    "start_time":"DAY1_00000000",
%    "query_time":"DAY4_17091712"}'
% }
% </tool>
% \end{verbatim}

% \end{tcolorbox}
